Leopard: Towards High Throughput-Preserving BFT for Large-scale Systems

With the emergence of large-scale decentralized applications, a scalable and efficient Byzantine Fault Tolerant (BFT) protocol of hundreds of replicas is desirable. Although the throughput of existing leader-based BFT protocols has reached a high level of $10^5$ requests per second for a small scale of replicas, it drops significantly when the number of replicas increases, which leads to a lack of practicality. This paper focuses on the scalability of BFT protocols and identifies a major bottleneck to leader-based BFT protocols due to the excessive workload of the leader at large scales. A new metric of scaling factor is defined to capture whether a BFT protocol will get stuck when it scales out, which can be used to measure the performance of efficiency and scalability of BFT protocols. We propose "Leopard", the first leader-based BFT protocol that scales to multiple hundreds of replicas, and more importantly, preserves a high efficiency. We remove the bottleneck by introducing a technique of achieving a constant scaling factor, which takes full advantage of the idle resource and adaptively balances the workload of the leader among all replicas. We implement Leopard and evaluate its performance compared to HotStuff, the state-of-the-art BFT protocol. We run extensive experiments on the two systems with up to 600 replicas. The results show that Leopard achieves significant performance improvements both on throughput and scalability. In particular, the throughput of Leopard remains at a high level of $10^5$ when the system scales out to 600 replicas. It achieves a $5\times$ throughput over HotStuff when the scale is 300 (which is already the largest scale we can see the progress of the latter in our experiments), and the gap becomes wider as the number of replicas further increases.

==> conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}
The scalability and efficiency are two key metrics for a practical BFT protocol. %, especially due to the emergence of decentralized applications. 
However, the throughput of most existing leader-based BFT protocols drops significantly as the scale increasing. They thus face a scalability-efficiency dilemma. In this paper, we analyzed the bottleneck to this problem and defined a new metric called ``scaling factor'' to capture whether a BFT protocol can preserve the efficiency when the number of replicas increases. We presented a leader-based BFT protocol called ``Leopard''.  Our protocol enables preserving high throughput when the scale grows. It obtains the ideal scaling factor that is constant to $n$, and supports a more effective scaling up with 1/2 improvement of throughput by doubling the configured bandwidth at each replica. This is achieved by amortizing the workload of the leader to other replicas and taking full advantage of the idle resources. We conducted a variety of experiments on the implementation of Leopard with up to 600 replicas. The evaluation shows the throughput of Leopard remains almost flat at $10^5$ and it achieves significant multi-sided performance improvements to the state-of-the-art BFT solution, HotStuff. 
%to get a constant scaling factor, which is the bottleneck of the protocol's efficiency and scalability. By taking full advantage of idle resources of other replicas, 

==> expdetail.tex <==
\section{Throughput on Varying the Batch Sizes}
\label{appendix:exp}

%\subsection{Experimental Results on Varying the Batch Sizes}
%\label{appendix:parameter}
%--------------------
In this section, we present experimental results on the measures of throughput with a varying batch size for both HotStuff and Leopard. The results are shown below. 

\begin{figure}[!h]
	\centering{\includegraphics[width=6cm]{Img/para/HotStuffPeak.eps}}
	\centering \caption{Throughput of HotStuff on varying batch sizes.}
	\label{fig:hotstuffpara}
\end{figure}

In HotStuff, there is only one batch for batching requests into a consensus proposal (i.e., a block). Fig. \ref{fig:hotstuffpara} depicts the throughput with different batch sizes for five replica numbers (32, 64, 128, 256, 300). Results show that the throughput goes up as we increasing the batch size, but it stops to grow after a certain batch size value. We let the batch size at this point be the implementation parameter of HotStuff. \tc{The latency, however, still goes up if we keeps increasing the batch size. }

%\begin{figure}[ht]
%	\centering		
%	\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/para/64-txb.eps}	
%	\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/para/64-bft.eps}	
%	\vspace{-2mm}
%	\caption{Performance of our system on varying batch sizes with $n=64$.}
%	\vspace{-2mm}
%	\label{fig:ourpara}
%\end{figure}

\begin{figure}[ht]
	\centering		
	\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/para/bftsize.eps}	
	\caption{Throughput of Leopard on varying batch sizes of a BFTblock.}
	\label{fig:ourparabft}
\end{figure}

\begin{figure}[!ht]
	\centering		
	\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/para/txbsize1.eps}	
	\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/para/txbsize2.eps}	
	\caption{Throughput of Leopard on varying datablock sizes with BFTblock size fixes at 10 (top) and 100 (bottom), respectively.}
	\label{fig:ourparatxb}
\end{figure}

In Leopard, there are two batch sizes, namely the BFTblock size and the datablock size. We varied one bath size while fixing the other one, to exam the effect on throughput. Fig. \ref{fig:ourparabft} depicts the throughput for six replica numbers (32 to 600) when the BFTblock size increases. It shows that, for all tested $n$, the upward trend of throughput has gradually stabilized as the BFTblock size increases. Generally, the size at which the throughput gets stabilized when $n$ is large is greater than the size when $n$ is small. It indicates that it requires a larger batch size in each agreement instance to amortize the increased cost caused by a larger $n$. We remark that, the peak throughput shown in Fig. \ref{fig:ourparabft} at different $n$ drops in Leopard. This is due to that, in this experiment, we fixed the datablock size for all tested $n$, whereas to preserve the throughput when $n$ increases, Leopard requires the datablock size (i.e., $\alpha$ in the analysis of $\S$\ref{section:analysis}) should increase when $n$ is getting larger. 
To exam the throughput when the datablock size increases, we choose two BFTblock sizes and see the result at different $n$. The result is shown in Fig. \ref{fig:ourparatxb}. Similar to the result on varying BFTblock sizes, it shows that for both BFTblock sizes and all tested $n$, the upward trend of throughput has also gradually stabilized as the datablock size increases. 





%
%\subsection{Analysis of the effectiveness when scaling up} 
%\label{appendix:cost-effectiveness}
%Now, we want to estimate how our protocol and existing leader-based BFT protocols, including HotStuff, perform when configuring with more bandwidth resources at each replica. We let $\Phi_\Delta$ denote the increased bits processed per second by the protocol, and $B_\Delta$ denote the increased bandwidth resources at each replica. Therefore, the rate of $\Phi_\Delta$ over $B_\Delta$ indicates the cost-effectiveness of the protocol. 
%
%As for existing leader-based protocols, we know from the analysis in $\S$\ref{section:intro} that, the leader gets stuck because an excessive workload on sending messages to other replicas. Following Eq. (\ref{Eq:sf_old}) in $\S$\ref{section:intro}, we have that, 
%\begin{equation}
%	(\frac{\Phi_\Delta}{B_\Delta})^\textrm{pre}=\frac{\Lambda_\Delta\times\textrm{payload}}{(\Gamma_\Delta)^\textrm{pre-send}_\textrm{leader}}=\frac{1}{n-1}.
%	\label{Eq:ce_old}
%\end{equation}
%It means that, the cost-effectiveness on the available bandwidth of existing leader-based BFT protocols drops at a rate of $\frac{1}{n-1}$. To confirm this, we recast the experimental result of HotStuff in Fig. \ref{fig:cost-effectiveness} and show it together with the theoretical result analyzed above in one figure. The result is depicted in Fig. \ref{fig:costE}. As we can see, the experimental result matches with the theoretical result above.
%
%\begin{figure}[ht]
%	\centering		
%	%\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/HotStuffBandwidthTPS.eps}	
%	\includegraphics[width=0.35\textwidth,trim=0 0 0 0,clip]{Img/HotStuffYieldRatio3.eps}	
%	\vspace{-2mm}
%	\caption{The cost-effectiveness of HotStuff with a varying $n$.}
%	\vspace{-2mm}
%	\label{fig:costE}
%\end{figure}
%
%As for our protocol and following Eq. (\ref{Eq:SF-ours}), when processing $\Lambda$ requests, it should configure about  $(2\cdot\textrm{payload}\times\Lambda)$ bandwidth at each replica assuming the parameter $\alpha$ is large enough. Hence, we have that,
%\begin{equation}
%	(\frac{\Phi_\Delta}{B_\Delta})^\textrm{ours}\approx\frac{\Lambda_\Delta\times\textrm{payload}}{2\cdot\textrm{payload}\times\Lambda_\Delta}=\frac{1}{2}.
%	\label{Eq:ce_ours}
%\end{equation}
%It means that, the cost-effectiveness on the available bandwidth of our protocol remains at about 1/2 for all scales. This is consistent with the evaluation result in Fig. \ref{fig:cost-effectiveness}.


%\subsection{Network Bandwidth Breakdown}
%\label{appendix:breakdown}
%
%To further evaluate the bandwidth usage at each replica in our system's implementation, we present a breakdown of bandwidth usages with $n=32$. The result is shown in Table \ref{table:bandwidth-breakdown}. 
%For the leader, most of bandwidth (over 96\%) was used on receiving datablocks from other $n-1$ replicas, whereas the second highest usage is from sending consensus proposals (about 3.17\%). 
%For each non-leader replica, most of the bandwidth is used on sending/receiving datablocks and the cost on sending is a little bit higher than the cost on receiving. This is due to that a replica sends a datablock to all $n-1$ others, but receives datablocks from $n-2$ other replicas (since the leader is excluded from generating the datablock). Notice that, the bandwidth used on receiving pending requests (both from other replicas and clients) takes up about 50\% of the total bandwidth usage at a non-leader replica. Since the achievable throughput is limited by the number of requests received per second, this indicates that the effective network bandwidth utilization ratio, i.e., confirmed bits per second over the configured bandwidth, is 1/2 in our protocol. %This is consistent with the evaluation result in Fig. \ref{fig:cost-effectiveness} (left figure).
%
%\renewcommand{\arraystretch}{1.2}
%\begin{table}[!h]
%	\centering
%	\caption{Network bandwidth usage breakdown of our system's implementation with $n=32$.}
%	\vspace{-2mm}
%	\footnotesize{
%		\begin{tabular}{|c|c|l||c|}	
%			\hline
%			Role & \multicolumn{2}{c||}{Usage} & \%Bandwidth\\
%			\hline\hline
%			\multirow{8}{*}{Leader}&\multirow{4}{*}{Sent}&Consensus Proposal& 3.17\%\\
%			&& Vote Result/Proof& 0.24\%\\
%			&&Miscellaneous & 0.15\%\\
%			\cline{3-4}
%			&&SUM & \textbf{3.56\%}\\
%			\cline{2-4}
%			&\multirow{4}{*}{Received}&Datablock& 96.17\%\\
%			&&Vote & 0.16\%\\
%			&&Miscellaneous& 0.10\%\\
%			\cline{3-4}
%			&&SUM &\textbf{96.44\%}\\
%			\hline			
%			\multirow{9}{*}{Non-leader}&\multirow{4}{*}{Sent}&Datablock& 49.93\%\\
%			&& Vote & 0.01\%\\
%			&&Miscellaneous& 0.05\%\\
%			\cline{3-4}
%			&&SUM & \textbf{49.99\%}\\
%			\cline{2-4}
%			&\multirow{5}{*}{Received}&Consensus Proposal& 0.05\%\\
%			Replica&&Datablock & 48.34\%\\
%			&&Vote Result/Proof& 0.01\%\\
%			&&Reqs. from Clients& 1.61\%\\
%			\cline{3-4}
%			&&SUM & \textbf{50.01\%}\\
%			\hline
%		\end{tabular}
%	}
%	\label{table:bandwidth-breakdown}
%	\vspace{-4mm}
%\end{table}





